Parameter-free Locality Sensitive Hashing for Spherical Range Reporting

We present a data structure for *spherical range reporting* on a point set $S$, i.e., reporting all points in $S$ that lie within radius $r$ of a given query point $q$. Our solution builds upon the Locality-Sensitive Hashing (LSH) framework of Indyk and Motwani, which represents the asymptotically best solutions to near neighbor problems in high dimensions. While traditional LSH data structures have several parameters whose optimal values depend on the distance distribution from $q$ to the points of $S$, our data structure is parameter-free, except for the space usage, which is configurable by the user. Nevertheless, its expected query time basically matches that of an LSH data structure whose parameters have been *optimally chosen for the data and query* in question under the given space constraints. In particular, our data structure provides a smooth trade-off between hard queries (typically addressed by standard LSH) and easy queries such as those where the number of points to report is a constant fraction of $S$, or where almost all points in $S$ are far away from the query point. In contrast, known data structures fix LSH parameters based on certain parameters of the input alone. The algorithm has expected query time bounded by $O(t (n/t)^\rho)$, where $t$ is the number of points to report and $\rho\in (0,1)$ depends on the data distribution and the strength of the LSH family used. We further present a parameter-free way of using multi-probing, for LSH families that support it, and show that for many such families this approach allows us to get expected query time close to $O(n^\rho+t)$, which is the best we can hope to achieve using LSH. The previously best running time in high dimensions was $\Omega(t n^\rho)$. For many data distributions where the intrinsic dimensionality of the point set close to $q$ is low, we can give improved upper bounds on the expected query time.

==> distributions.tex <==
\subsection{Structured Inputs with Large Gaps}
In many real-world data sets \cite{?} there is a gap between the true nearest neighbors of a query and 
points that are far away. Here we assume that the number of points that are not far away from 
the real close points of a query is bounded by the number of close points in the radius of
$r + 1, \ldots, cr$ for a constant $c > 1$. The following Corollary shows that Algorithm~\ref{algo:adaptive:query}
gives strong running time guarantees in this setting.

\begin{corollary}
Let $S \subseteq \{0,1\}^d$ with $|S| = n$ and $r$ be given, and assume that 
the data structure has been set up with parameters $k$ and $L$. Let $q \in \{0,1\}^d$ be the query point.  
Suppose there exists a constant $c$ such that there are $t$ close points at distance at most
$r$, and the number of points at distance between $r$ and $cr$ is at most $\Theta(t)$. If $k \geq 
\log (n/t) / \log (1/(1 - cr/d))$, 
Algorithm~\ref{algo:adaptive:query} returns each close point with constant probability 
in expected runnting time 
$O\left(t\cdot \left(n/t\right)^\rho\right).$
\label{cor:input:with:gaps}
\end{corollary}

Before we prove the corollary we want to point out that the value of $k$ is always at most the
k parameter 
needed to solve the $(r,cr)$-nearest neighbor problem with traditional LSH. However, the 
time bounds are much better than in this case. So, we get data- and output-sensitivity 
\emph{for free}. 

\begin{proof}[Proof of Corollary~\ref{cor:input:with:gaps}.]
If $k = \log (n/t)/ \log (1/p_2)$ is probed, we get the desired bounds.
\end{proof}



\subsection{Gamma Distribution}



